The Way to my Heart is through Contrastive Learning: Remote Photoplethysmography from Unlabelled Video

The ability to reliably estimate physiological signals from video is a powerful tool in low-cost, pre-clinical health monitoring. In this work we propose a new approach to remote photoplethysmography (rPPG) - the measurement of blood volume changes from observations of a person's face or skin. Similar to current state-of-the-art methods for rPPG, we apply neural networks to learn deep representations with invariance to nuisance image variation. In contrast to such methods, we employ a fully self-supervised training approach, which has no reliance on expensive ground truth physiological training data. Our proposed method uses contrastive learning with a weak prior over the frequency and temporal smoothness of the target signal of interest. We evaluate our approach on four rPPG datasets, showing that comparable or better results can be achieved compared to recent supervised deep learning methods but without using any annotation. In addition, we incorporate a learned saliency resampling module into both our unsupervised approach and supervised baseline. We show that by allowing the model to learn where to sample the input image, we can reduce the need for hand-engineered features while providing some interpretability into the model's behavior and possible failure modes. We release code for our complete training and evaluation pipeline to encourage reproducible progress in this exciting new direction.

==> tables/channel-in.tex <==
\textbf{Input channels}
\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{footnotesize}
\begin{tabular}{llccccccc}
\toprule
Method & Dataset & R & G & B & RG & RB & GB & RGB \\
\midrule
Sup. & COHFACE & 8.8 & 2.2 & 8.7 & 2.1 & 8.0 & 2.0 & 2.0 \\
 & PURE & 20.5 & 2.4 & 2.4 & 2.5 & 2.2 & 2.4 & 2.2 \\
 & UBFC & 5.9 & 2.9 & 2.4 & 2.9 & 2.5 & 2.9 & 2.9 \\
\cmidrule{2-9}
 & Mean & 11.7 & 2.5 & 4.5 & 2.5 & 4.3 & 2.4 & 2.4 \\
\midrule
Cont. & COHFACE & 18.4 & 11.0 & 13.4 & 9.3 & 13.8 & 14.8 & 5.3 \\
 & PURE & 23.1 & 2.1 & 2.3 & 2.2 & 2.0 & 2.3 & 2.2 \\
 & UBFC & 47.6 & 2.9 & 30.7 & 2.9 & 28.5 & 28.9 & 2.9 \\
\cmidrule{2-9}
 & Mean & 29.7 & 5.3 & 15.5 & 4.8 & 14.8 & 15.4 & 3.5 \\
\bottomrule
\end{tabular}
\end{footnotesize}
}
\end{center}
\caption{\textbf{Effect of input channel combinations on test-set heart rate RMSE.} Performance on unseen test subjects per dataset for supervised and contrastive approaches. Agreement with domain knowledge that Green channel is most information for rPPG due to absorption spectrum. Supervised models can do reasonable well on all inputs except Red channel only. Our contrastive approach benefits from access to all input channels, particularly for more heavily compressed data (COHFACE). Why?}
\label{table:channelin}
\end{table}

==> tables/cohface.tex <==
\begin{table}
\begin{footnotesize}
\begin{center}
\begin{tabular}{lcccccc}


\toprule
 & \multicolumn{3}{c}{Heart Rate} & \multicolumn{2}{c}{PPG Signal} \\
 & RMSE & MAE & PC & Corr & MCC \\
\midrule
Mean & 15.41 & 12.08 & -0.18 & -0.01 & 0.14 \\
Median & 15.43 & 12.09 & -0.15 & -0.01 & 0.14 \\
\midrule
HR-CNN & 10.74 & 8.10 & 0.29 &  &  \\
\midrule
Our Supervised & 5.11 & 1.54 & 0.89 & -0.16 & 0.65 \\
Contrast (NMCC) & 3.34 & 1.01 & 0.95 & 0.39 & 0.71 \\
Contrast (PSD MSE) & 2.99 & 0.94 & 0.96 & 0.17 & 0.72 \\
\bottomrule


\end{tabular}
\end{center}
\caption{\textbf{Results on COHFACE~\cite{} dataset.}}
\end{footnotesize}
\end{table}

==> tables/mirl.tex <==
\begin{table}
\begin{footnotesize}
\begin{center}
\begin{tabular}{lcccccc}


\toprule
 & \multicolumn{3}{c}{Heart Rate} & \multicolumn{2}{c}{PPG Signal} \\
 & RMSE & MAE & PC & Corr & MCC \\
\midrule
Mean & 16.61 & 14.21 & - & -0.02 & 0.31 \\
Median & 17.90 & 15.77 & - & 0.01 & 0.25 \\
\midrule
AutoSparsePPG & 2.90 &  &  &  &  \\
\midrule
Our Supervised & 2.24 & 0.85 & 0.96 & 0.40 & 0.77 \\
Contrast (NMCC) & 1.38 & 0.65 & 0.98 & -0.32 & 0.70 \\
Contrast (PSD MSE) & 1.73 & 0.73 & 0.98 & -0.59 & 0.72 \\
\bottomrule


\end{tabular}
\end{center}
\caption{\textbf{Results on MR-NIRP-Car~\cite{} dataset.}}
\end{footnotesize}
\end{table}

==> tables/pure.tex <==

\begin{table}
\begin{footnotesize}
\begin{center}
\begin{tabular}{lccc@{\hskip 0.25in}cc}


\toprule
 & \multicolumn{3}{c}{Heart Rate} & \multicolumn{2}{c}{PPG Signal} \\
 & RMSE & MAE & PC & Corr & MCC \\
\midrule
Mean & 16.14 & 13.21 & -0.14 & 0.00 & 0.10 \\
Median & 23.97 & 21.15 & -0.16 & 0.00 & 0.07 \\
\midrule
HR-CNN & 2.37 & 1.84 & 0.98 &  &  \\
\midrule
Supervised & 2.38 & 1.91 & 0.99 & 0.57 & 0.84 \\
Contrast (NMCC) & 2.28 & 1.81 & 0.99 & 0.21 & 0.75 \\
Contrast (PSD MSE) & 2.53 & 2.02 & 0.99 & -0.38 & 0.79 \\
\bottomrule


\end{tabular}
\end{center}
\caption{\textbf{Results on PURE~\cite{stricker2014non} dataset.}}
\end{footnotesize}
\end{table}



==> tables/ubfc.tex <==
\begin{table}
\begin{footnotesize}
\begin{center}
\begin{tabular}{lcccccc}


\toprule
 & \multicolumn{3}{c}{Heart Rate} & \multicolumn{2}{c}{PPG Signal} \\
 & RMSE & MAE & PC & Corr & MCC \\
\midrule
Mean & 19.44 & 16.58 & -0.14 & 0.01 & 0.10 \\
Median & 19.45 & 16.58 & -0.22 & 0.02 & 0.10 \\
\midrule
Meta-rPPG & 7.42 & 5.97 & 0.53 &  &  \\
\midrule
Our Supervised & 4.71 & 3.52 & 0.95 & 0.18 & 0.64 \\
Contrast (NMCC) & 4.34 & 3.38 & 0.95 & -0.32 & 0.61 \\
Contrast (PSD MSE) & 4.39 & 3.44 & 0.95 & -0.36 & 0.63 \\
\bottomrule


\end{tabular}
\end{center}
\caption{\textbf{Results on UBFC~\cite{} dataset.}}
\end{footnotesize}
\end{table}
